CharXiv: Charting Gaps in Realistic Chart Understanding in Multimodal LLMs

Chart understanding plays a pivotal role when applying Multimodal Large Language Models (MLLMs) to real-world tasks such as analyzing scientific papers or financial reports. However, existing datasets often focus on oversimplified and homogeneous charts with template-based questions, leading to an over-optimistic measure of progress. We demonstrate that although open-source models can appear to outperform strong proprietary models on these benchmarks, a simple stress test with slightly different charts or questions can deteriorate performance by up to 34.5%. In this work, we propose CharXiv, a comprehensive evaluation suite involving 2,323 natural, challenging, and diverse charts from arXiv papers. CharXiv includes two types of questions: 1) descriptive questions about examining basic chart elements and 2) reasoning questions that require synthesizing information across complex visual elements in the chart. To ensure quality, all charts and questions are handpicked, curated, and verified by human experts. Our results reveal a substantial, previously underestimated gap between the reasoning skills of the strongest proprietary model (i.e., GPT-4o), which achieves 47.1% accuracy, and the strongest open-source model (i.e., InternVL Chat V1.5), which achieves 29.2%. All models lag far behind human performance of 80.5%, underscoring weaknesses in the chart understanding capabilities of existing MLLMs. We hope CharXiv facilitates future research on MLLM chart understanding by providing a more realistic and faithful measure of progress. Project page and leaderboard: https://charxiv.github.io/

==> sections/checklist.tex <==
\newpage
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} 
    
    \green{All contents are substantiated by \cref{sec:motivation,,sec:charxiv_overview,,sec:experiments}.}
  \item Did you describe the limitations of your work?
    \answerYes{} 
    
    \green{We provide limitations in \cref{lim_and_impacts}}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} 
    
    \green{We provide potential negative societal impacts in \cref{lim_and_impacts}}.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}

    \green{We carefully read the guidelines and ensured that the submission conforms to them.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}

    \green{We do not have theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}

    \green{We do not have theoretical results.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}

    \green{We include the codebase and link to data in the supplementary material. Instructions to reproduce main experimental results are present in \cref{tab:run_configurations}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{} 
    
    \green{We do not train models. We provide splits of the benchmark in \cref{sec:charxiv_overview} and the hyperparamters of the evaluations in \cref{tab:run_configurations}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)? \answerNA{}
 
    \green{We use fixed parameters to generate deterministic model responses (whenever possible) in our benchmark, which we provide details in \cref{tab:run_configurations}}.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{} 
    
    \green{We only evaluate the models, so we do not provide information on compute in a separate section. Regardless, all open-source models are evaluated on either a single A100 or H100 GPU from minutes to hours. We use API to evaluate proprietary models.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}

    \green{Our metadata contains information that can be used to trace back to the original assets.}
  \item Did you mention the license of the assets?
    \answerYes{}

    \green{License for preprints on arXiv server is publicly available \href{https://info.arxiv.org/help/license/index.html}{online}. We provide license information for models we evaluate in \cref{tab:model_license}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
    
    \green{We provide 60 samples of our annotated data in \cref{sec:desc_failure} and \cref{sec:reas:failure}. Our codebase and annotated data can be found in \url{https://charxiv.github.io}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}

    \green{We adhere to applicable license regulations on arXiv. All questions and answers are new assets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}

    \green{Every individual chart and question has gone through human inspections and our data do not contain any personally identifiable information or offensive content, except for proper attribution to the source of the charts.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}

    \green{Our general guidelines are elaborated in \cref{sec:charxiv_overview}. We provide screenshots of annotations in \cref{subsec:chart_selection_annotation,,subsec:descriptive_q_annotation,,subsec:reasoning_q_annotation}}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}

    \green{We did not recruit external human subjects in our study}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}

    \green{We did not recruit external human subjects in our study}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
